Analysis of Corrected Graph Convolutions

Machine learning for node classification on graphs is a prominent area driven by applications such as recommendation systems. State-of-the-art models often use multiple graph convolutions on the data, as empirical evidence suggests they can enhance performance. However, it has been shown empirically and theoretically, that too many graph convolutions can degrade performance significantly, a phenomenon known as oversmoothing. In this paper, we provide a rigorous theoretical analysis, based on the two-class contextual stochastic block model (CSBM), of the performance of vanilla graph convolution from which we remove the principal eigenvector to avoid oversmoothing. We perform a spectral analysis for $k$ rounds of corrected graph convolutions, and we provide results for partial and exact classification. For partial classification, we show that each round of convolution can reduce the misclassification error exponentially up to a saturation level, after which performance does not worsen. We also extend this analysis to the multi-class setting with features distributed according to a Gaussian mixture model. For exact classification, we show that the separability threshold can be improved exponentially up to $O({\log{n}}/{\log\log{n}})$ corrected convolutions.

==> my-preamble.tex <==
% ams packages
\usepackage{amsmath, amssymb, amsthm}

% biblatex
\usepackage[style=alphabetic]{biblatex}
\appto{\bibsetup}{\sloppy}
\bibliography{references}

% other packages
\usepackage{algorithm}
\usepackage{algorithmic}

\usepackage{enumitem}
\usepackage{framed}
\usepackage{xcolor}
\usepackage{bbm} % \mathbbm{1}
\usepackage{ulem} % for sout needs it

% Table of contents with links
\usepackage{color}
\usepackage{hyperref}
\hypersetup{
    colorlinks = true,
    linktoc = all,
    linkcolor = blue
}

% The demon that is called tikz...
\usepackage{tikz}
\usetikzlibrary{arrows.meta}

\usepackage{graphicx}
\usepackage{caption}
\usepackage{subcaption}

\usepackage{verbatim}

% page layout and spacing setting
\makeatletter
  \setlength{\textwidth}{6.5in}
  \setlength{\oddsidemargin}{0in}
  \setlength{\evensidemargin}{0in}
  \setlength{\topmargin}{0.25in}
  \setlength{\textheight}{8.25in}
  \setlength{\headheight}{0pt}
  \setlength{\headsep}{0pt}
  \setlength{\marginparwidth}{59pt}

  \setlength{\parindent}{0pt}
% \setlength{\parskip}{3pt}
  \setlength{\parskip}{5pt plus 1pt}
% \setlength{\theorempreskipamount}{5pt plus 1pt}
% \setlength{\theorempostskipamount}{0pt}
  \setlength{\abovedisplayskip}{8pt plus 3pt minus 6pt}
\makeatother

% theorem etc. setting
% [theorem] means numbering is the same as theorem
\newtheorem{theorem}{Theorem}[section]
\newtheorem{definition}[theorem]{Definition}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{corollary}[theorem]{Corollary}

\newtheorem{assumption}[theorem]{Assumption}
\newtheorem{claim}[theorem]{Claim}
\newtheorem{conjecture}[theorem]{Conjecture}
\newtheorem{example}[theorem]{Example}
\newtheorem{fact}[theorem]{Fact}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{question}[theorem]{Question}

\newtheorem{problem}[theorem]{Problem}
\newtheorem*{problem*}{Problem}
\newtheorem{remark}[theorem]{Remark}
\newtheorem*{remark*}{Remark}
\makeatletter
\DeclareRobustCommand{\cev}[1]{%
  {\mathpalette\do@cev{#1}}%
}
\newcommand{\do@cev}[2]{%
  \vbox{\offinterlineskip
    \sbox\z@{$\m@th#1 x$}%
    \ialign{##\cr
      \hidewidth\reflectbox{$\m@th#1\vec{}\mkern4mu$}\hidewidth\cr
      \noalign{\kern-\ht\z@}
      $\m@th#1#2$\cr
    }%
  }%
}
\makeatother
% math notation
\newcommand{\R}{\ensuremath{\mathbb R}}
\newcommand{\C}{\ensuremath{\mathbb C}}
\newcommand{\Z}{\ensuremath{\mathbb Z}}
\newcommand{\N}{\ensuremath{\mathbb N}}
\renewcommand{\H}{\ensuremath{\mathbb H}} % upper half plane
\renewcommand{\S}{\ensuremath{\mathbb S}} % sphere

\newcommand{\E}{\ensuremath{\mathbb E}}
\newcommand{\Hess}{\ensuremath{\mathcal H}}
\newcommand{\eps}{\ensuremath{\varepsilon}}
\newcommand{\Lcirc}{\ensuremath{\mathring{L}}} % for Lorentzian polynomials
\renewcommand{\emptyset}{\ensuremath{\varnothing}}

\newcommand{\ceil}[1]{\ensuremath{\left\lceil#1\right\rceil}}
\newcommand{\floor}[1]{\ensuremath{\left\lfloor#1\right\rfloor}}
\newcommand{\norm}[1]{\ensuremath{\left\lVert#1\right\rVert}}

\renewcommand{\Re}{\operatorname{Re}}
\renewcommand{\Im}{\operatorname{Im}}
\DeclareMathOperator{\Arg}{Arg}
\DeclareMathOperator{\tr}{tr}
\DeclareMathOperator{\polylog}{polylog}
\newcommand{\sleq}{\preccurlyeq}
\newcommand{\sgeq}{\succcurlyeq}


\DeclareMathOperator{\diag}{diag}
\DeclareMathOperator{\supp}{supp}
\DeclareMathOperator{\conv}{conv}
\DeclareMathOperator{\Var}{Var}
\DeclareMathOperator{\Inf}{Inf}
\newcommand{\one}{\ensuremath{\mathbbm{1}}}
\newcommand{\Fil}{\mathcal{F}} % filtration

% colors
\newcommand{\red}[1]{\textcolor{red}{#1}}
\newcommand{\green}[1]{\textcolor{green}{#1}}

% convex programs
\DeclareMathOperator{\st}{subject~to}

% hyphen
\mathchardef\mhyphen="2D

\newcommand{\directed}{\ensuremath{\overrightarrow}}

% horizontal dash in matrix
\makeatletter
\newcommand{\longdash}[1][2em]{%
  \makebox[#1]{$\m@th\smash-\mkern-7mu\cleaders\hbox{$\mkern-2mu\smash-\mkern-2mu$}\hfill\mkern-7mu\smash-$}}
\makeatother
\newcommand{\omitskip}{\kern-\arraycolsep}
\newcommand{\llongdash}[1][2em]{\longdash[#1]\omitskip}
\newcommand{\rlongdash}[1][2em]{\omitskip\longdash[#1]}
  
% inner product
\newcommand{\inner}[2]{\ensuremath{\langle #1, #2 \rangle}}

% math in tabular
\usepackage{array}   % for \newcolumntype macro
\newcolumntype{C}{>{$}c<{$}}

% Tikz stuff
\newcommand{\solidcircle}{\tikz\draw[black,fill=black] (0,0) circle (.5ex);}
\newcommand{\hollowcircle}{\tikz\draw[black,fill=white] (0,0) circle (.5ex);}
